Adversarial Graph Augmentation to Improve Graph Contrastive Learning

Self-supervised learning of graph neural networks (GNN) is in great need because of the widespread label scarcity issue in real-world graph/network data. Graph contrastive learning (GCL), by training GNNs to maximize the correspondence between the representations of the same graph in its different augmented forms, may yield robust and transferable GNNs even without using labels. However, GNNs trained by traditional GCL often risk capturing redundant graph features and thus may be brittle and provide sub-par performance in downstream tasks. Here, we propose a novel principle, termed adversarial-GCL (AD-GCL), which enables GNNs to avoid capturing redundant information during the training by optimizing adversarial graph augmentation strategies used in GCL. We pair AD-GCL with theoretical explanations and design a practical instantiation based on trainable edge-dropping graph augmentation. We experimentally validate AD-GCL by comparing with the state-of-the-art GCL methods and achieve performance gains of up-to $14\%$ in unsupervised, $6\%$ in transfer, and $3\%$ in semi-supervised learning settings overall with 18 different benchmark datasets for the tasks of molecule property regression and classification, and social network classification.

==> section_tex_files/results.tex <==
\input{tables/unsupervised_tu_dataset_results}

==> section_tex_files/theory.tex <==
In this section, we demonstrate the theoretical insights behind 


\subsection{Multi-View Formulation}

\pan{Theorem: Consider the following optimization problem
\begin{align}
    \max_{f\in \mathcal{F}}\min_{t\in \mathcal{T}} I(f(G), f(t(G))) 
\end{align}
Consider two levels of views 
\begin{enumerate}
    \item Good view: $t(G)$ such that $t(G) \perp_{Y} G$. That is, we have the Markov chain $G \rightarrow Y \rightarrow t(G)$.
    %\item [Optimal view] Good view + $$
    \item Optimal view: $t(G)$ such that $t(G) \perp_{Y} G$. For all $t(G)\in \mathcal{T}$, $I(t(G), Y) = I(G, Y)$.
\end{enumerate}
%If $ t\in \mathcal{T}$ such that $t(G) \perp_{Y} G$, which forms the Markov chain $G \rightarrow Y \rightarrow t(G)$ and we call its good view, then 
If $\mathcal{T}$ contains a good view, then,
\begin{align}
    \max_{f\in \mathcal{F}}\min_{t\in \mathcal{T}} I(f(G), f(t(G))) \leq \max_{f\in \mathcal{F}} I(f(G), Y). 
\end{align}
If $\mathcal{T}$ contains an optimal view and $\mathcal{F}$ contains a bijective encoder, then,
\begin{align}
    \max_{f\in \mathcal{F}}\min_{t\in \mathcal{T}} I(f(G), f(t(G))) = \max_{f\in \mathcal{F}} I(f(G), Y) = I(G,Y). 
\end{align}
}

We first start with the InfoMax principle \citep{linsker1988self} for representation learning, which suggests to choose a representation that maximizes the mutual information (MI) between the input and its representation. Formally, for input $G$ and a function class $\mathcal{F}$ of the encoder, the InfoMax objective is, \pan{$G\sim \mathcal{D}$, where $\mathcal{D}$ is a distribution.} \sus{Yes}

\begin{equation}
\label{eq:infomax}
    \max_{f \in \mathcal{F}} I(G;f(G))
\end{equation}

Instead of maximizing MI in the original high dimensional data space, MI can also be maximized between representations of two \textit{views} of the original data. 
\pan{Define views?}

\sus{How to formally define them ? I was thinking ... First draw two augmentation functions $t_{1} \sim \mathcal{T}$ and $t_{2} \sim \mathcal{T}$ and then set $G^{1} = t_{1}(G)$ and $G^{2} = t_{2}(G)$. $\mathcal{T}$ represents the augmentation pool. }


\begin{equation}
\label{eq:multi_view}
    \max_{f_{1} \in \mathcal{F}_{1}, f_{2} \in \mathcal{F}_{2}} I \Big(f_{1} (G^{1}) ; f_{2} (G^{2})\Big)
\end{equation}

\begin{equation}
\label{eq:multi_view}
    \max_{f \in \mathcal{F}}\min_{t\in \mathcal{T}} I \Big(f(G) ; f (t(G))\Big)
\end{equation}

\begin{equation}
\label{eq:multi_view}
    I \Big(G ; f(G)\Big) \leq I \Big( (G,f(G)) ; f(G)\Big) = I\Big( G ; f(G) | f(G)\Big) + I\Big( f(G) ; f(G)\Big) = I\Big( f(G) ; f(G)\Big) 
\end{equation}
$\max_{f} I\Big( f(G) ; f(G)\Big)$

Our objective:
\begin{equation}
\label{eq:multi_view}
    \max_{f \in \mathcal{F}}\min_{t\in \mathcal{T}} I \Big(f(G) ; f (t(G))\Big)
\end{equation}
If we do not have a control on $\mathcal{T}$, the above optimization will give us trivial solutions. 

We define that $\mathcal{T}$ as to preturb the edges in the the input graphs. Suppose it input is $G=(V,E)$. For the edge $e\in E$, the dropout prob is $p_e$. We constrain $\mathcal{T}$ as for $t\in \mathcal{T}$ that in $t(G)$, $\sum_{e\in E} p_e \leq k * |E|$. 

Change the objective as 
\begin{equation}
\label{eq:multi_view}
    \max_{f \in \mathcal{F}}\min_{t\in \mathcal{T}} E_G(-nce-loss + \lambda \sum_{e\in E} p_e/|E|)) 
\end{equation}

where, $I$ is the MI which is usually estimated, $G^{1}$ and $G^{2}$ are the different views of $G$, for instance: rotations or cropping in the image domain and node dropping or edge perturbation in the graph domain. $f_{1}$ and $f_{2}$ can share parameters and their function classes provide modelling flexibility.
\pan{If $f_1$ and $f_2$ share parameters, they are the same model. Why do we use different subscripts and different ambient spaces $F_1$ and $F_2$? I guess $f_1$ and $f_2$ are just the same encoder. }

\sus{They "may" or "may not" share parameters. It depends on the implementation. So, I write the two encoders separately to be as general as possible.}

It can be shown that objective in Eq.~\ref{eq:multi_view} is a lower bound of the original InfoMax objective. The proof follows a standard application of chain rule for mutual information.

\begin{proposition}
\label{prop:multi_view}
For a given random variable $G$ and two augmented views $G^{1} = t_{1}(G), G^{2} = t_{2}(G)$ generated by arbitrary augmentation functions $t_{1}$ and $t_2$ then, $I(G^{1}; G^{2}) \leq I\big(G ; (G^{1}, G^{2}) \big)$. \pan{Is this your contribution?} 

\sus{While the multi-view formulation is know, the connection is usually loosely said in previous work. I include the proposition to make things clear later on and for completeness. The mult-iview formulation is based on \cite{tschannen2019mutual}. Our proof is also easy to see rather than using markov chains as done by \cite{tschannen2019mutual}. While this doesn't have to be in the main text. It can go to the supplement.}
\end{proposition}
\begin{proof}
Firstly, using the chain rule of MI in two different ways we expand,
\begin{align}
\label{eq:prop1_1}
  I\big(G^{1} ; (G, G^{2})\big) &= I(G^{1} ; G) + I(G^{1}; G^{2}| G) \\
  &= I(G^{1} ; G^{2}) + I(G^1; G | G^{2})
\end{align}

Since, $G^{1}$ and $G^{2}$ are conditionally independent given $G$ i.e. $(G^{1} \bigCI G^{2}) | G$ by definition \pan{So we need to claim that two views inject independent randomness in the proposition statement} we have $I(G^{1}; G^{2}| G) = 0$.
\begin{equation}
    \label{eq:prop1_2}
    I(G^{1} ; G) = I(G^{1} ; G^{2}) + I(G^1; G | G^{2})
\end{equation}
By non-negativity of MI, in (\ref{eq:prop1_2}), we have, $I(G^1; G | G^{2})) \geq 0$. Thus,
\begin{equation}
    \label{eq:prop1_3}
    I(G^{1} ; G) \geq I(G^{1} ; G^{2})
\end{equation}

Another application of chain rule and non negativity of MI leads to,
\begin{equation}
    \label{eq:prop1_4}
    I\big(G; (G^{1}, G^{2})\big) = I(G;G^{1}) + I(G; G^{2} | G^{1}) \\
    \geq I(G;G^{1})
\end{equation}
Lastly from (\ref{eq:prop1_3}) and (\ref{eq:prop1_4}) we have, $I(G^{1}; G^{2}) \leq I\big(G ; (G^{1}, G^{2}) \big)$
\end{proof}
\pan{Just for a note to see how loose this bound would be \\ $ I(G, f(G)) \geq I\big(G ; (f(G^{1}), f(G^{2}))) = I\big(G ; f(G^{1})) + I\big(G; f(G^{2}) | f(G^{1})) = I\big(f(G^{1}); f(G^{2})) + I\big(f(G^{1}); G|f(G^{2})) + I\big(G; f(G^{2}) | f(G^{1})) $}

\begin{corollary}
In particular, for MI between encoded representations of the views we have, $I(f_{1}(G^{1}); f_{2}(G^{2})) \leq I\big(G ; (f_{1}(G^{1}), f_{2}(G^{2})) \big) \leq I(G, f(G))$
\end{corollary}
This connects the multi-view formulation to the InfoMax principle.

\paragraph{Critical choices} The choice of views, encoders and the kind of MI estimation all play a crucial role in the behaviour of the objective in Eq.~\ref{eq:multi_view}. While the role of the MI estimator and encoders have been studied before \cite{} leading to multiple methods, views are usually hand designed heuristically through data augmentation and there is a lack of studies especially in the graph domain.

\subsection{Contrastive Learning (CL)}
It stems from the use of InfoNCE ($I_{\text{NCE}}$) objective \cite{} used to estimate MI in Eq.~\ref{eq:multi_view}. Formally, for random variables $G^{1}$ and $G^{2}$ representing views of data $G$, the goal of this paradigm is to learn a parameterized function that can distinguish between samples drawn from the empirical joint distribution $p(G^{1}, G^{2})$ and samples drawn from the product of marginals $p(G^{1})p(G^{2})$. \pan{This is because $I(G^{1}, G^{2}) = KL(p(G^{1}, G^{2})|| p(G^{1}) p(G^{2})) )$ } This is done by defining the InfoNCE loss as,
\begin{equation}
\label{eq:info_nce_loss}
    \mathcal{L}_{\text{NCE}}(G^{1}, G^{2}) = -\mathbb{E}\Bigg[ \log \frac{e^{h(G^{1}_{i}, G^{2}_{i})}}{\sum_{j=1}^{K} e^{h(G^{1}_{i}, G^{2}_{j})}} \Bigg]
\end{equation}
Sample $G_i \sim \mathcal{D}$
\pan{Be rigorous: what is the expectation here to compute. We are mixing population representation and empirical representation. }
\sus{The expectation is over all anchor points in the batch.}
where, $G^{1}_{i}$ is the anchor point and minimizing the above loss function favours scoring the positives $G^{2}_{i} \sim p(G^{2} | G^{1}_{i})$ higher compared to a set of K negatives ${G^{2}_j \sim p(G^{2}); \forall j=1 \cdots K}$. The score function $h(\cdot , \cdot)$ can take on different forms and the most common one is the cosine similarity of the encoded representations. The exact form will be shown later in the implementation.

It has been shown that minimizing $\mathcal{L}_{\text{NCE}}$ infact maximizes a lower bound of mutual information between the two views termed $I_{\text{NCE}}$.
\begin{equation}
    I(G^{1}, G^{2}) \geq \log(K) - \mathcal{L}_{\text{NCE}}(G^{1}, G^{2}) \triangleq I_{\text{NCE}}(G^{1}, G^{2})
\end{equation}

\subsection{Influence of Views}

\begin{figure}
    \centering
    \includegraphics[width=0.2\textwidth]{figures/multi_view_graphical_model.png}
    \caption{Simplified Multi-View Graphical Model}
    \label{fig:graphical_model}
\end{figure}
We now study the effect of using views for the CL objective, consider the graphical model as shown in Fig.~\ref{fig:graphical_model}. For our analysis we simplify view $G^{1}$ as the original input $G$ itself and view $G^{2}$ as its augmented version $G^{v} = t(G)$. The augmentation is done by first sampling a function $t \sim \mathcal{T}$. 

To characterize the quality of the representations learned in the CL paradigm, they are evaluated on a separate downstream task $\mathcal{Y}$. Thus, we include the task information $Y$ in the graphical model for such analysis, but it should be noted that for contrastive learning of representations, task/label information is not used.

Now for a generic multiclass classification task, we define,

% \begin{wrapfigure}[5]{r}{0.2\textwidth} 
%     \centering
%     \includegraphics[width=0.2\textwidth]{figures/multi_view_graphical_model.pdf}
%     \caption{Caption}
%     \label{fig:my_label}
% \end{wrapfigure}

\pan{This is not the definition of the error?}

\sus{I get this definition from \cite{feder1994relations}. It is the error made by the \textbf{best possible estimator} of $Y$ based on the knowledge of $Z$. Practically, it is in line with how representations are evaluated. After learning $Z$ (by inturn learning parameters of $f$ using CL), a linear classifier is used for downstream task. }

\sus{The reason for choosing this kind of minimal ideal error is that, if we can get a upper bound on it's behaviour, it can \textbf{suggest} how empirical estimator error will behave }

\begin{definition}[Minimal Error Probability]
Consider the task of predicting $Y$ from the learned representation $Z = f(G)$ in CL paradigm. Let $\hat{Y}$ be the estimate of $Y$. The minimum probability of error in estimating $Y$ given observation $z$ of $Z$ is the MAP estimator $\hat{y} = \argmax_{y} P(Y=y|Z=z)$. The expected minimal error probability is then, 
\begin{equation}
    \pi = \mathbb{E}_{z} [1 - \max_{y} P(Y=y|Z=z)]
\end{equation}
\end{definition}

% \begin{theorem}[Lower Bound of Error Probability - Fano's Inequality \citep{fano1961transmission}]

% \end{theorem}

\begin{theorem}[Upper Bound of Minimal Error Probability \citep{feder1994relations}]
\label{thm:error_upper_bound}
The expected minimal error probability of estimation can be upper bounded in terms of conditional entropy as, 
\[\pi \leq 1 - e^{-H(Y|Z)}\]
\end{theorem}
\begin{theorem}[Minimal Error Probability and Contrastive Learning]
\[\pi \leq 1 - \exp\Big(-\big[H(Y) - I(Z; Z^{v}) + I(G; G^{v}) + I(G^{v}; Y | G) - I(G^{v} ; Y)
+ I(Z;G|G^{v},Y)\big]\Big)\]

\end{theorem}
\begin{proof}
We first start with the result in Thm.~\ref{thm:error_upper_bound} and write the conditional entropy in terms of mutual information. So,
\begin{equation}
    \label{eq:thm2_0}
    \pi \leq 1 - e^{-[H(Y) - I(Z;Y)]}
\end{equation}
We now seek to understand the term $I(Z;Y)$.

Using chain rule of MI we can expand,
\begin{align}
    I(Z;(G,Y)) &= I(Z,G) + I(Z;Y|G) \\
    &= I(Z;Y) + I(Z;G|Y)
\end{align}
Now, $I(Z;Y|G) = 0$ as $Z = f(G)$ and $f$ is deterministic (\pan{I will go back to this point.}). So, from above we have,
\begin{equation}
    \label{eq:thm2_1}
    I(Z;Y) = I(Z;G) - I(Z;G | Y)
\end{equation}

Similarly, 
\begin{align}
    I(Z; (G, Z^{v})) &= I(Z;G) + I(Z;Z^{v}|G) \\
    &= I(Z;Z^{v}) + I(Z;G|Z^{v})
\end{align} \pan{$Z^v$ has not been defined.}

\sus{It is in the graphical model. Figure~\ref{fig:graphical_model}}

Again, $I(Z;Z^{v}|G) = 0$. Thus,
\begin{equation}
    \label{eq:thm2_2}
    I(Z;G) = I(Z;Z^{v}) + I(Z;G|Z^{v})
\end{equation}
Using (\ref{eq:thm2_2}) in (\ref{eq:thm2_1}) we get, 
\begin{align}
    I(Z;Y) &= I(Z;Z^{v}) + I(Z;G|Z^{v}) - I(Z;G | Y)\\
     &\geq I(Z;Z^{v}) - I(Z;G | Y) \label{eq:thm2_3}
\end{align}
by non-negativity of MI i.e. $I(Z;G|Z^{v}) \geq 0$. 

Further chain rule allows us to write,
\begin{align}
    I(Z;(G,G^{v}) | Y) &= I(Z;G|Y) + I(Z;G^{v} | G,Y) \\
    &= I(Z;G^{v} | Y) + I(Z;G| G^{v}, Y)
\end{align}
Since $I(Z;G^{v} | G,Y) = 0$, we get,
\begin{equation}
    \label{eq:thm2_4}
    I(Z;G|Y) = I(Z;G^{v} | Y) + I(Z;G| G^{v}, Y)
\end{equation}
Using (\ref{eq:thm2_4}) in (\ref{eq:thm2_3}) we get,
\begin{equation}
    \label{eq:thm2_5}
    I(Z;Y) \geq I(Z;Z^{v}) - I(Z;G^{v} | Y) - I(Z;G| G^{v}, Y)
\end{equation}

From the Data Processing Inequality \citep{cover1999elements}, as $Z = f(G)$, we know functions of data cannot increase MI. Thus,
\begin{equation}
    \label{eq:thm2_6}
    I(Z; G^{v} | Y) \leq I(G ; G^{v} | Y)
\end{equation}
From (\ref{eq:thm2_5}) and (\ref{eq:thm2_6}) we get,
\begin{equation}
    \label{eq:thm2_7}
    I(Z;Y) \geq I(Z;Z^{v}) - I(G ; G^{v} | Y) - I(Z;G| G^{v}, Y)
\end{equation}

Further we expand,
\begin{align}
    I(G^{v};(G,Y)) &= I(G^{v};G) + I(G^{v};Y|G) \\
    &= I(G^{v} ; Y) + I(G^{v} ; G | Y)
\end{align}
From above, 
\begin{equation}
    \label{eq:thm2_8}
    I(G^{v} ; G | Y) = I(G^{v};G) + I(G^{v};Y|G) - I(G^{v} ; Y)
\end{equation}
Using (\ref{eq:thm2_8}) in (\ref{eq:thm2_7}) we get,
\begin{equation}
    \label{eq:thm2_9}
    I(Z;Y) \geq I(Z;Z^{v}) - I(G^{v};G) - I(G^{v};Y|G) + I(G^{v} ; Y) - I(Z;G| G^{v}, Y)    
\end{equation}

Finally, we finish the proof by using (\ref{eq:thm2_9}) in (\ref{eq:thm2_0}) to obtain,
\begin{equation}
    \pi \leq 1 - \exp\Big(-\big[H(Y) - I(Z; Z^{v}) + I(G; G^{v}) + I(G^{v}; Y | G) - I(G^{v} ; Y)
+ I(Z;G|G^{v},Y)\big]\Big)
\end{equation}
\end{proof}

The above theorem throws light on some important properties of the contrastive learning paradigm. Firstly, it states that the error probability $\pi$ is low ($\downarrow$) when
\begin{enumerate}
    \item $I(Z; Z^{v})$ is high ($\uparrow$). Maximizing MI between representations of the two view is beneficial. This aligns with the popular multi-view InfoMax principle (see Prop ~\ref{prop:multi_view}).
    \item $I(G^{v} ; Y)$ is high ($\uparrow$). Select view that maintains high mutual information with the downstream task. 
    \item $I(G; G^{v})$ is low ($\downarrow$). Select views that share minimal MI with each other.
    \item $I(G^{v}; Y | G)$ is low ($\downarrow$). Extra task relevant information in view should be minimal. \pan{This is 0?}
    \sus{That is the best case. It will be high if the task is tailored to the view $G^{v}$ and not depend much on the original data. This will usually be the noise $G^{v}$ shares with $Y$ and we want it to be minimal.}
    \item $I(Z;G|G^{v},Y)$ is low ($\downarrow$). We can understand this term better if we look at Eq.~\ref{eq:thm2_4}. This term is the redundant information i.e. $I(Z;G|Y) - I(Z;G^{v}|Y)$. For this to be low, we would want $Z$'s to be similar for the views. Explain more.
    \item $H(Y)$ is some constant. It depends on the task.
\end{enumerate}

Only performing point 1. is not enough as done in standard contrastive learning. Point 5. is kind of taken care is we use the same encoder for both views. And the similarity metric $h(\cdot, \cdot)$ in InfoNCE loss Eq.~\ref{eq:info_nce_loss} aligns with this point. Empirically also SimCLR does this and gets SOTA results in image classification. 

Point 2, 3 and 4 are usually hand designed by carefully choosing the kinds of view.



\paragraph{Note: \todo{}} Just as we derived the relation between error probability and CL in the classification task setting, we can also relate minimum mean squared error (a.k.a. MMSE) and CL in the regression task setting. This makes use of Tao's inequality and results from Verdu \url{(http://www.stat.yale.edu/~yw562/reprints/mmse_functional.pdf}.





==> tables/unsupervised_results_biochem.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[htb]
\centering
\renewcommand{\arraystretch}{1.5}
\newcommand{\STAB}[1]{\begin{tabular}{@{}c@{}}#1\end{tabular}}
\resizebox{0.6\textwidth}{!}{%
\begin{tabular}{clcccc}
\hline
& Dataset                                      & NCI1           & PROTEINS            & MUTAG          & DD \\ \hline

& F-GIN & 78.27 $\pm$ 1.35 & 72.39 $\pm$ 2.76 & 90.41 $\pm$ 4.61 & 74.87 $\pm$ 3.56 \\ \hline
\multirow{3}{*}{\STAB{\rotatebox[origin=c]{90}{Baselines}}}& RU-GIN~\cite{xu2018how}& 62.98 $\pm$ 0.10 & 69.03 $\pm$ 0.33 & 87.61 $\pm$ 0.39 & 74.22 $\pm$ 0.30  \\
& InfoGraph~\cite{sun2019infograph}& 68.13 $\pm$ 0.59 & 72.57 $\pm$ 0.65 & 87.71 $\pm$ 1.77 & 75.23 $\pm$ 0.39\\
& GraphCL ~\cite{you2020graph}& 68.54 $\pm$ 0.55 & 72.86 $\pm$ 1.01 & 88.29 $\pm$ 1.31 & 74.70 $\pm$ 0.70\\\hline
\multirow{2}{*}{\STAB{\rotatebox[origin=c]{90}{AB-S}}}& NAD-GCL-FIX & 69.23 $\pm$ 0.60 & 72.81 $\pm$ 0.71 & 88.58 $\pm$ 1.58 & 74.55 $\pm$ 0.55\\
& NAD-GCL-OPT & 69.30 $\pm$ 0.32 & 73.18 $\pm$ 0.71 & 89.05 $\pm$ 1.06 & 74.55 $\pm$ 0.55\\\hline\hline
\multirow{2}{*}{\STAB{\rotatebox[origin=c]{90}{Ours}}} 

& AD-GCL-FIX & \bf{69.67 $\pm$ 0.51}$^\star$ & \bf{73.59 $\pm$ 0.65} & \bf{89.25 $\pm$ 1.45} & 74.49 $\pm$ 0.52\\ 

& AD-GCL-OPT & \bf{69.67 $\pm$ 0.51}$^\star$ & \bf{73.81 $\pm$ 0.46}$^\star$ & \textbf{89.70 $\pm$ 1.03} & 75.10 $\pm$ 0.39\\ \hline\hline
\end{tabular}%
}
\caption{Supplement the results of Table~\ref{tab:dataset-stats-tu-unsup}: Unsupervised Learning performance for biochemical graph classification in TU datasets (Averaged accuracy $\pm$ std. over 10 runs). \textbf{Bold}/\textbf{Bold}$^\star$ indicats our methods outperform baselines with $\geq$ 0.5/$\geq$ 2 std respectively. Fully supervised (F-GIN) results are shown \textbf{only} for placing GRL methods in perspective. Ablation-study (AB-S) results do not count as baselines.}
\label{tab:unsupervised_learning_biochem}
\end{table}

==> tables/unsupervised_results_social.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[t]
\centering
\renewcommand{\arraystretch}{1.5}
\newcommand{\STAB}[1]{\begin{tabular}{@{}c@{}}#1\end{tabular}}
\resizebox{\textwidth}{!}{%
\begin{tabular}{clccccccccc}
\hline
& Dataset                                      & NCI1           & PROTEINS            & MUTAG          & DD                                      & COLLAB           & RDT-B            & RDT-M5K          & IMDB-B           & IMDB-M           \\ \hline

& F-GIN & 78.27 $\pm$ 1.35 & 72.39 $\pm$ 2.76 & 90.41 $\pm$ 4.61 & 74.87 $\pm$ 3.56 & 74.82 $\pm$ 0.92 & 86.79 $\pm$ 2.04 & 53.28 $\pm$ 3.17 & 71.83 $\pm$ 1.93 & 48.46 $\pm$ 2.31 \\ \hline
\multirow{3}{*}{\STAB{\rotatebox[origin=c]{90}{Baselines}}}&RU-GIN~\cite{xu2018how}& 62.98 $\pm$ 0.10 & 69.03 $\pm$ 0.33 & 87.61 $\pm$ 0.39 & 74.22 $\pm$ 0.30  & 63.08 $\pm$ 0.10 & 58.97 $\pm$ 0.13 & 27.52 $\pm$ 0.61 & 51.86 $\pm$ 0.33 & 32.81 $\pm$ 0.57 \\
& InfoGraph~\cite{sun2019infograph}& 68.13 $\pm$ 0.59 & 72.57 $\pm$ 0.65 & 87.71 $\pm$ 1.77 & 75.23 $\pm$ 0.39                                     & 70.35 $\pm$ 0.64 & 78.79 $\pm$ 2.14 & 51.11 $\pm$ 0.55 & 71.11 $\pm$ 0.88 & 48.66 $\pm$ 0.67 \\
& GraphCL ~\cite{you2020graph}& 68.54 $\pm$ 0.55 & 72.86 $\pm$ 1.01 & 88.29 $\pm$ 1.31 & 74.70 $\pm$ 0.70                                     & 71.26 $\pm$ 0.55 & 82.63 $\pm$ 0.99 & 53.05 $\pm$ 0.40 & 70.80 $\pm$ 0.77 & 48.49 $\pm$ 0.63 \\\hline
\multirow{2}{*}{\STAB{\rotatebox[origin=c]{90}{AB-S}}}& NAD-GCL-FIX & 69.23 $\pm$ 0.60 & 72.81 $\pm$ 0.71 & 88.58 $\pm$ 1.58 & 74.55 $\pm$ 0.55              & 71.56 $\pm$ 0.58 & 83.41 $\pm$ 0.66 & 52.72 $\pm$ 0.71 & 70.94 $\pm$ 0.77 & 48.33 $\pm$ 0.47 \\
& NAD-GCL-OPT & 69.30 $\pm$ 0.32 & 73.18 $\pm$ 0.71 & 89.05 $\pm$ 1.06 & 74.55 $\pm$ 0.55             & 72.04 $\pm$ 0.67 & 83.74 $\pm$ 0.76 & 53.43 $\pm$ 0.26 & 71.94 $\pm$ 0.59 & 49.01 $\pm$ 0.93 \\\hline\hline
\multirow{2}{*}{\STAB{\rotatebox[origin=c]{90}{Ours}}} 

& AD-GCL-FIX & \bf{69.67 $\pm$ 0.51}$^\star$ & \bf{73.59 $\pm$ 0.65} & \bf{89.25 $\pm$ 1.45} & 74.49 $\pm$ 0.52 & \textbf{73.32 $\pm$ 0.61}$^\star$ & \textbf{85.52 $\pm$ 0.79}$^\star$ & \textbf{53.00 $\pm$ 0.82} & \textbf{71.57 $\pm$ 1.01} & \textbf{49.04 $\pm$ 0.53} \\ 

& AD-GCL-OPT & \bf{69.67 $\pm$ 0.51}$^\star$ & \bf{73.81 $\pm$ 0.46}$^\star$ & \textbf{89.70 $\pm$ 1.03} & 75.10 $\pm$ 0.39 & \textbf{73.32 $\pm$ 0.61}$^\star$ & \textbf{85.52 $\pm$ 0.79}$^\star$ & \textbf{54.93 $\pm$ 0.43}$^\star$ & \textbf{72.33 $\pm$ 0.56}$^\star$ & \textbf{49.89 $\pm$ 0.66}$^\star$ \\ \hline\hline
\end{tabular}%
}
\caption{\small{Unsupervised Learning performance for social network classification (Averaged accuracy $\pm$ std. over 10 runs). \textbf{Bold} indicates our methods outperform baselines with $\geq$ 0.5 std.. \textbf{Bold}$^\star$ indicates our methods outperform baselines with $\geq$ 2 std.. Fully supervised (F-GIN) results are shown \textbf{only} for placing GRL methods in perspective. Ablation-study (AB-S) results do not count as baselines.} }
\label{tab:unsupervised_learning_social}
\end{table}

==> tables/unsupervised_tu_dataset_results.tex <==
% % Please add the following required packages to your document preamble:
% % \usepackage{booktabs}
% \begin{table}[b]
% \begin{tabular}{@{}lllllllll@{}}
% \toprule
%                                                                      & NCI1 & PROTEINS & DD & MUTAG & COLLAB & RDT-B & RDT-M5K & IMDB-B \\ \midrule
% \begin{tabular}[c]{@{}l@{}}No Train \\ (Encoder GIN)\end{tabular}    &      &          &    &       &        &       &         &        \\
% InfoGraph                                                            &      &          &    &       &        &       &         &        \\
% \begin{tabular}[c]{@{}l@{}}GraphCL \\ (Identical Views)\end{tabular} &      &          &    &       &        &       &         &        \\
% GraphCL                                                              &      &          &    &       &        &       &         &        \\
% Ours - InfoMinMax                                                    &      &          &    &       &        &       &         &        \\
%                                                                      &      &          &    &       &        &       &         &        \\ \bottomrule
% \end{tabular}
% \caption{}
% \label{tab:my-table}
% \end{table}


